A New Achievable Rate Region for Multiple-Access Channel with States

The problem of reliable communication over the multiple-access channel (MAC) with states is investigated. We propose a new coding scheme for this problem which uses quasi-group codes (QGC). We derive a new computable single-letter characterization of the achievable rate region. As an example, we investigate the problem of doubly-dirty MAC with modulo-$4$ addition. It is shown that the sum-rate $R_1+R_2=1$ bits per channel use is achievable using the new scheme. Whereas, the natural extension of the Gel'fand-Pinsker scheme, sum-rates greater than $0.32$ are not achievable.

==> MATH_template.tex <==
\usepackage{tikz}
%\usepackage{mathdots}
\usepackage[utf8]{inputenc}

\usepackage{mathrsfs}
\usepackage{amsmath} \usepackage{amsthm} \usepackage{amsfonts} \usepackage{amssymb} 
\usepackage{epstopdf}
%\usepackage{mathtools}
\usepackage{graphicx}
%\usepackage{relsize}
%\usepackage{xy}
\input{xypic}
\usepackage{bbm}
%\setlength{\footskip}{20pt}

\usepackage{enumerate}

%\onecolumn

%\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lem}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{definition}{Definition}

\theoremstyle{definition}
\newtheorem{example}{Example}
\newtheorem{conjecture}{Conjecture}
\newtheorem{question}{Question}
\newtheorem{problem}{Problem}
\newtheorem*{prob*}{Problem}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{rems}{Remarks}
\newtheorem{para}{}
\newtheorem{summary}{Summary}



\renewcommand{\Re}[1]{\ensuremath{\operatorname{Re}\left\{#1\right\}}}
\renewcommand{\Im}[1]{\ensuremath{\operatorname{Im}\left\{#1\right\}}}

\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}

\global\long\def\Z{\mathrm{{\bf Z}}}
\global\long\def\N{\mathrm{{\bf N}}}
\global\long\def\Gal{\mathrm{Gal}}





\global\long\def\RR{\mathbb{R}}
\global\long\def\CC{\mathbb{C}}
\global\long\def\NN{\mathbb{N}}
\global\long\def\QQ{\mathbb{Q}}
\global\long\def\ZZ{\mathbb{Z}}
\global\long\def\EE{\mathbb{E}}
\global\long\def\PP{\mathbb{P}}
\global\long\def\FF{\mathbb{F}}

 \global\long\def\dd{\cdots}
\global\long\def\normal{\triangleleft}

\newcommand*{\Scale}[2][4]{\scalebox{#1}{\ensuremath{#2}}}%
